Exploring compactified HEIDI models at the LHC

Models with multi-scalar Higgs sectors inspired by a higher-dimensional setup are interesting alternatives to the Standard Model because, although they have a Higgs sector which gives mass to the W and Z gauge bosons as well as the SM fermions, this Higgs sector is potentially undiscoverable at the Large Hadron Collider or shows considerable deviations from the Standard Model Higgs sector. We investigate a compactified version of such models and study its phenomenology in the "golden" four-lepton channel at the LHC in areas of parameter space compatible with electroweak precision observables.

==> table_mhm.tex <==
\begin{tabular}{|lcl|l|lllllll|l|}
\hline & & & & \multicolumn{7}{|c|}{\sc FeynRules} & \multicolumn{1}{|c|}{Stock}\\
\multicolumn{3}{|c|}{Process} & \multicolumn{1}{|c|}{$\sqrt{s}$}
 & \multicolumn{1}{|c}{MG} & \multicolumn{1}{c}{CH} & \multicolumn{1}{c}{WO2}
 & \multicolumn{1}{c}{WO1} & \multicolumn{1}{c}{WO1} & \multicolumn{1}{c}{CH}
 & \multicolumn{1}{c|}{WO2} & \multicolumn{1}{|c|}{WO2}\\
& & & \multicolumn{1}{c}{\scriptsize[GeV]} & \multicolumn{1}{|c}{U}
 & \multicolumn{1}{c}{U} & \multicolumn{1}{c}{U} & \multicolumn{1}{c}{F}
 & \multicolumn{1}{c}{U} & \multicolumn{1}{c}{F} & \multicolumn{1}{c|}{F}
 & \multicolumn{1}{|c|}{U}\\
\hline\hline
$\scriptstyle g\;g$ & $\scriptstyle\rightarrow$ & $\scriptstyle g\;g$ &
 $\scriptstyle 200$ 
 & {\scriptsize 1.88e04} & {\scriptsize 1.88e04} & {\scriptsize 1.88e04}
 & {\scriptsize 1.88e04} & {\scriptsize 1.88e04} & {\scriptsize 1.88e04}
 & {\scriptsize 1.88e04} & {\scriptsize 1.88e04}
\\
$\scriptstyle Z\;W^+$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle {Z}^\prime\;{W^+}^\prime$ & $\scriptstyle 4693$ 
 & {\scriptsize 103} & {\scriptsize 103} & {\scriptsize 103} & {\scriptsize 103}
 & {\scriptsize 103} & {\scriptsize 103} & {\scriptsize 103} & {\scriptsize 103}
\\
$\scriptstyle \gamma\;\gamma$ & $\scriptstyle\rightarrow$ & $\scriptstyle W^+\;W^-$ &
 $\scriptstyle 643$ 
 & {\scriptsize 16.1} & {\scriptsize 16.1} & {\scriptsize 16.1} & {\scriptsize 16.1}
 & {\scriptsize 16.1} & {\scriptsize 16.1} & {\scriptsize 16.1} & {\scriptsize 16.1}
\\
$\scriptstyle Z\;W^+$ & $\scriptstyle\rightarrow$ & $\scriptstyle W^+\;{Z}^\prime$ &
 $\scriptstyle 3015$ 
 & {\scriptsize 0.755} & {\scriptsize 0.755} & {\scriptsize 0.755} & {\scriptsize 0.755}
 & {\scriptsize 0.755} & {\scriptsize 0.755} & {\scriptsize 0.755} & {\scriptsize 0.756}
\\
$\scriptstyle \gamma\;Z$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle {W^+}^\prime\;{W^-}^\prime$ & $\scriptstyle 8730$ 
 & {\scriptsize 0.0412} & {\scriptsize 0.0412} & {\scriptsize 0.0411}
 & {\scriptsize 0.0412} & {\scriptsize 0.0412} & {\scriptsize 0.0412}
 & {\scriptsize 0.0412} & {\scriptsize 0.0412}
\\
$\scriptstyle \gamma\;Z$ & $\scriptstyle\rightarrow$ & $\scriptstyle W^+\;{W^-}^\prime$ &
 $\scriptstyle 2686$ 
 & {\scriptsize 1.30} & {\scriptsize 1.30} & {\scriptsize 1.30} & {\scriptsize 1.30}
 & {\scriptsize 1.30} & {\scriptsize 1.30} & {\scriptsize 1.30} & {\scriptsize 1.30}
\\
$\scriptstyle W^+\;{W^+}^\prime$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle {W^+}^\prime\;{W^+}^\prime$ & $\scriptstyle 6322$ 
 & {\scriptsize 3.32} & {\scriptsize 3.31} & {\scriptsize 3.31} & {\scriptsize 3.31}
 & {\scriptsize 3.31} & {\scriptsize 3.31} & {\scriptsize 3.31} & {\scriptsize 3.32}
\\
$\scriptstyle Z\;{Z}^\prime$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle {W^+}^\prime\;{W^-}^\prime$ & $\scriptstyle 6371$ 
 & {\scriptsize 3.86} & {\scriptsize 3.86} & {\scriptsize 3.86} & {\scriptsize 3.86}
 & {\scriptsize 3.86} & {\scriptsize 3.86} & {\scriptsize 3.86} & {\scriptsize 3.86}
\\
$\scriptstyle W^+\;W^+$ & $\scriptstyle\rightarrow$ & $\scriptstyle W^+\;{W^+}^\prime$ &
 $\scriptstyle 2965$ 
 & {\scriptsize 2.41} & {\scriptsize 2.42} & {\scriptsize 2.42} & {\scriptsize 2.42}
 & {\scriptsize 2.42} & {\scriptsize 2.42} & {\scriptsize 2.42} & {\scriptsize 2.42}
\\
$\scriptstyle \gamma\;W^+$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle {Z}^\prime\;{W^+}^\prime$ & $\scriptstyle 8656$ 
 & {\scriptsize 0.0349} & {\scriptsize 0.0349} & {\scriptsize 0.0349}
 & {\scriptsize 0.0349} & {\scriptsize 0.0349} & {\scriptsize 0.0349}
 & {\scriptsize 0.0349} & {\scriptsize 0.0349}
\\\hline
$\scriptstyle W^+\;{W^-}^\prime$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle s\;{\bar{s}}^\prime$ & $\scriptstyle 18765$ 
 & {\scriptsize 33.6} & {\scriptsize 33.6} & {\scriptsize 33.6} & {\scriptsize 33.6}
 & {\scriptsize 33.6} & {\scriptsize 33.6} & {\scriptsize 33.6} & {\scriptsize 33.6}
\\
$\scriptstyle {Z}^\prime\;{Z}^\prime$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle b\;\bar{b}$ & $\scriptstyle 8094$ 
 & {\scriptsize 0.0958} & {\scriptsize 0.0959} & {\scriptsize 0.0959}
 & {\scriptsize 0.0959} & {\scriptsize 0.0959} & {\scriptsize 0.0959}
 & {\scriptsize 0.0959} & {\scriptsize 0.0959}
\\
$\scriptstyle {Z}^\prime\;{Z}^\prime$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle {e^-}^\prime\;{e^+}^\prime$ & $\scriptstyle 36900$ 
 & {\scriptsize 1.54} & {\scriptsize 1.54} & {\scriptsize 1.54} & {\scriptsize 1.54}
 & {\scriptsize 1.54} & {\scriptsize 1.54} & {\scriptsize 1.54} & {\scriptsize 1.54}
\\
$\scriptstyle \gamma\;{W^+}^\prime$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle {c}^\prime\;{\bar{s}}^\prime$ & $\scriptstyle 34886$ 
 & {\scriptsize 0.00220} & {\scriptsize 0.00220} & {\scriptsize 0.00220}
 & {\scriptsize 0.00220} & {\scriptsize 0.00220} & {\scriptsize 0.00220}
 & {\scriptsize 0.00220} & {\scriptsize 0.00220}
\\
$\scriptstyle W^+\;{W^-}^\prime$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle {\tau^-}^\prime\;{\tau^+}^\prime$ & $\scriptstyle 35208$ 
 & {\scriptsize 1.45} & {\scriptsize 1.45} & {\scriptsize 1.45} & {\scriptsize 1.45}
 & {\scriptsize 1.45} & {\scriptsize 1.45} & {\scriptsize 1.45} & {\scriptsize 1.45}
\\
$\scriptstyle W^+\;{W^-}^\prime$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle u\;{\bar{u}}^\prime$ & $\scriptstyle 18765$ 
 & {\scriptsize 34.0} & {\scriptsize 34.0} & {\scriptsize 34.0} & {\scriptsize 34.0}
 & {\scriptsize 34.0} & {\scriptsize 34.0} & {\scriptsize 34.0} & {\scriptsize 34.0}
\\
$\scriptstyle Z\;Z$ & $\scriptstyle\rightarrow$ & $\scriptstyle u\;{\bar{u}}^\prime$ &
 $\scriptstyle 17173$ 
 & {\scriptsize 30.3} & {\scriptsize 30.3} & {\scriptsize 30.3} & {\scriptsize 30.3}
 & {\scriptsize 30.3} & {\scriptsize 30.3} & {\scriptsize 30.3} & {\scriptsize 30.3}
\\
$\scriptstyle {W^+}^\prime\;{W^-}^\prime$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle b\;{\bar{b}}^\prime$ & $\scriptstyle 20460$ 
 & {\scriptsize 38.5} & {\scriptsize 38.5} & {\scriptsize 38.5} & {\scriptsize 38.5}
 & {\scriptsize 38.5} & {\scriptsize 38.5} & {\scriptsize 38.5} & {\scriptsize 38.4}
\\
$\scriptstyle {W^+}^\prime\;{W^-}^\prime$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle {\nu_e}^\prime\;{\bar{\nu}_e}^\prime$ & $\scriptstyle 36886$ 
 & {\scriptsize 1.64} & {\scriptsize 1.64} & {\scriptsize 1.64} & {\scriptsize 1.64}
 & {\scriptsize 1.64} & {\scriptsize 1.64} & {\scriptsize 1.64} & {\scriptsize 1.64}
\\
$\scriptstyle \gamma\;\gamma$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle {\mu^-}^\prime\;{\mu^+}^\prime$ & $\scriptstyle 32886$ 
 & {\scriptsize 0.000463} & {\scriptsize 0.000463} & {\scriptsize 0.000463}
 & {\scriptsize 0.000463} & {\scriptsize 0.000463} & {\scriptsize 0.000463}
 & {\scriptsize 0.000463} & {\scriptsize 0.000463}
\\\hline
$\scriptstyle \nu_\tau\;u$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle {\nu_\tau}^\prime\;{u}^\prime$ & $\scriptstyle 32886$ 
 & {\scriptsize 0.0966} & {\scriptsize 0.0966} & {\scriptsize 0.0967}
 & {\scriptsize 0.0966} & {\scriptsize 0.0966} & {\scriptsize 0.0966}
 & {\scriptsize 0.0966} & {\scriptsize 0.0966}
\\
$\scriptstyle \nu_e\;u$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle {\nu_e}^\prime\;{u}^\prime$ & $\scriptstyle 32886$ 
 & {\scriptsize 0.0966} & {\scriptsize 0.0966} & {\scriptsize 0.0966}
 & {\scriptsize 0.0966} & {\scriptsize 0.0966} & {\scriptsize 0.0966}
 & {\scriptsize 0.0967} & {\scriptsize 0.0967}
\\
$\scriptstyle c\;\bar{c}$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle {\nu_e}^\prime\;{\bar{\nu}_e}^\prime$ & $\scriptstyle 32896$ 
 & {\scriptsize 5.38e-06} & {\scriptsize 5.38e-06} & {\scriptsize 5.38e-06}
 & {\scriptsize 5.38e-06} & {\scriptsize 5.38e-06} & {\scriptsize 5.38e-06}
 & {\scriptsize 5.38e-06} & {\scriptsize 5.38e-06}
\\
$\scriptstyle b\;{u}^\prime$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle {t}^\prime\;{d}^\prime$ & $\scriptstyle 49606$ 
 & {\scriptsize 0.0337} & {\scriptsize 0.0337} & {\scriptsize 0.0337}
 & {\scriptsize 0.0337} & {\scriptsize 0.0337} & {\scriptsize 0.0337}
 & {\scriptsize 0.0337} & {\scriptsize 0.0337}
\\
$\scriptstyle \tau^-\;\bar{d}$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle {\nu_\tau}^\prime\;{\bar{u}}^\prime$ & $\scriptstyle 32893$ 
 & {\scriptsize 0.386} & {\scriptsize 0.386} & {\scriptsize 0.386} & {\scriptsize 0.386}
 & {\scriptsize 0.386} & {\scriptsize 0.386} & {\scriptsize 0.386} & {\scriptsize 0.386}
\\
$\scriptstyle e^-\;b$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle {e^-}^\prime\;{b}^\prime$ & $\scriptstyle 32903$ 
 & {\scriptsize 0.0965} & {\scriptsize 0.0965} & {\scriptsize 0.0965}
 & {\scriptsize 0.0965} & {\scriptsize 0.0965} & {\scriptsize 0.0965}
 & {\scriptsize 0.0966} & {\scriptsize 0.0965}
\\
$\scriptstyle t\;{\bar{\nu}_\tau}^\prime$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle {\tau^+}^\prime\;{b}^\prime$ & $\scriptstyle 50014$ 
 & {\scriptsize 0.0430} & {\scriptsize 0.0429} & {\scriptsize 0.0429}
 & {\scriptsize 0.0429} & {\scriptsize 0.0429} & {\scriptsize 0.0429}
 & {\scriptsize 0.0429} & {\scriptsize 0.0429}
\\
$\scriptstyle c\;\bar{s}$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle {\nu_e}^\prime\;{e^+}^\prime$ & $\scriptstyle 32892$ 
 & {\scriptsize 1.82e-05} & {\scriptsize 1.82e-05} & {\scriptsize 1.82e-05}
 & {\scriptsize 1.82e-05} & {\scriptsize 1.82e-05} & {\scriptsize 1.82e-05}
 & {\scriptsize 1.82e-05} & {\scriptsize 1.82e-05}
\\
$\scriptstyle \nu_\tau\;\bar{\nu}_\tau$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle t\;{\bar{t}}^\prime$ & $\scriptstyle 17388$ 
 & {\scriptsize 7.23e-06} & {\scriptsize 7.24e-06} & {\scriptsize 7.24e-06}
 & {\scriptsize 7.24e-06} & {\scriptsize 7.24e-06} & {\scriptsize 7.24e-06}
 & {\scriptsize 7.24e-06} & {\scriptsize 7.24e-06}
\\
$\scriptstyle \tau^-\;\tau^+$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle s\;{\bar{s}}^\prime$ & $\scriptstyle 16458$ 
 & {\scriptsize 9.33e-06} & {\scriptsize 9.35e-06} & {\scriptsize 9.35e-06}
 & {\scriptsize 9.35e-06} & {\scriptsize 9.35e-06} & {\scriptsize 9.35e-06}
 & {\scriptsize 9.35e-06} & {\scriptsize 9.35e-06}
\\\hline
\end{tabular}


==> table_mssm.tex <==
\begin{tabular}{|lcl|l|llll|ll|}
\hline & & & & \multicolumn{4}{|c|}{\sc FeynRules} & \multicolumn{2}{|c|}{Stock}\\
\multicolumn{3}{|c|}{Process} & \multicolumn{1}{|c|}{$\sqrt{s}$}
 & \multicolumn{1}{|c}{CH} & \multicolumn{1}{c}{MG} & \multicolumn{1}{c}{WO1}
 & \multicolumn{1}{c|}{WO2} & \multicolumn{1}{|c}{MG} & \multicolumn{1}{c|}{WO2}\\
& & & \multicolumn{1}{c}{\scriptsize[GeV]} & \multicolumn{1}{|c}{U}
 & \multicolumn{1}{c}{U} & \multicolumn{1}{c}{U} & \multicolumn{1}{c|}{U}
 & \multicolumn{1}{|c}{U} & \multicolumn{1}{c|}{U}\\
\hline\hline
$\scriptstyle Z\;Z$ & $\scriptstyle\rightarrow$ & $\scriptstyle W^+\;W^-$ &
 $\scriptstyle 1368$ 
 & {\scriptsize 26.2} & {\scriptsize 26.3} & {\scriptsize 26.2} & {\scriptsize 26.2}
 & {\scriptsize 26.3} & {\scriptsize 26.2}
\\
$\scriptstyle W^+\;W^+$ & $\scriptstyle\rightarrow$ & $\scriptstyle W^+\;W^+$ &
 $\scriptstyle 1277$ 
 & {\scriptsize 25.6} & {\scriptsize 25.7} & {\scriptsize 25.6} & {\scriptsize 25.7}
 & {\scriptsize 25.7} & {\scriptsize 25.6}
\\
$\scriptstyle \gamma\;Z$ & $\scriptstyle\rightarrow$ & $\scriptstyle W^+\;W^-$ &
 $\scriptstyle 1003$ 
 & {\scriptsize 19.3} & {\scriptsize 19.3} & {\scriptsize 19.3} & {\scriptsize 19.3}
 & {\scriptsize 19.3} & {\scriptsize 19.3}
\\
$\scriptstyle g\;g$ & $\scriptstyle\rightarrow$ & $\scriptstyle g\;g$ &
 $\scriptstyle 800$ 
 & {\scriptsize 839} & {\scriptsize 840} & {\scriptsize 839} & {\scriptsize 839}
 & {\scriptsize 839} & {\scriptsize 839}
\\
$\scriptstyle Z\;Z$ & $\scriptstyle\rightarrow$ & $\scriptstyle Z\;Z$ &
 $\scriptstyle 1459$ 
 & {\scriptsize 0.223} & {\scriptsize 0.223} & {\scriptsize 0.223} & {\scriptsize 0.223}
 & {\scriptsize 0.223} & {\scriptsize 0.223}
\\
$\scriptstyle \gamma\;\gamma$ & $\scriptstyle\rightarrow$ & $\scriptstyle W^+\;W^-$ &
 $\scriptstyle 1278$ 
 & {\scriptsize 4.95} & {\scriptsize 4.96} & {\scriptsize 4.95} & {\scriptsize 4.95}
 & {\scriptsize 4.96} & {\scriptsize 4.95}
\\\hline
$\scriptstyle \widetilde{g}\;\widetilde{g}$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle g\;g$ & $\scriptstyle 4862$ 
 & {\scriptsize 0.977} & {\scriptsize 0.977} & {\scriptsize 0.977} & {\scriptsize 0.977}
 & {\scriptsize 0.977} & {\scriptsize 0.977}
\\
$\scriptstyle \tau^-\;\tau^+$ & $\scriptstyle\rightarrow$ & $\scriptstyle \gamma\;Z$ &
 $\scriptstyle 758$ 
 & {\scriptsize 0.327} & {\scriptsize 0.327} & {\scriptsize 0.327} & {\scriptsize 0.327}
 & {\scriptsize 0.327} & {\scriptsize 0.327}
\\
$\scriptstyle \widetilde{\chi}^0_4\;\widetilde{\chi}_1^+$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle \gamma\;W^+$ & $\scriptstyle 2573$ 
 & {\scriptsize 0.0219} & {\scriptsize 0.0219} & {\scriptsize 0.0219}
 & {\scriptsize 0.0219} & {\scriptsize 0.0219} & {\scriptsize 0.0219}
\\
$\scriptstyle d\;\bar{d}$ & $\scriptstyle\rightarrow$ & $\scriptstyle Z\;Z$ &
 $\scriptstyle 730$ 
 & {\scriptsize 0.0838} & {\scriptsize 0.0839} & {\scriptsize 0.0838}
 & {\scriptsize 0.0838} & {\scriptsize 0.0839} & {\scriptsize 0.0839}
\\
$\scriptstyle t\;\bar{t}$ & $\scriptstyle\rightarrow$ & $\scriptstyle g\;g$ &
 $\scriptstyle 1400$ 
 & {\scriptsize 6.00} & {\scriptsize 6.00} & {\scriptsize 6.00} & {\scriptsize 5.99}
 & {\scriptsize 6.00} & {\scriptsize 5.99}
\\
$\scriptstyle c\;\bar{c}$ & $\scriptstyle\rightarrow$ & $\scriptstyle \gamma\;\gamma$ &
 $\scriptstyle 800$ 
 & {\scriptsize 0.0272} & {\scriptsize 0.0272} & {\scriptsize 0.0272}
 & {\scriptsize 0.0272} & {\scriptsize 0.0272} & {\scriptsize 0.0272}
\\
$\scriptstyle b\;\bar{b}$ & $\scriptstyle\rightarrow$ & $\scriptstyle W^+\;W^-$ &
 $\scriptstyle 678$ 
 & {\scriptsize 1.72} & {\scriptsize 1.72} & {\scriptsize 1.72} & {\scriptsize 1.72}
 & {\scriptsize 1.72} & {\scriptsize 1.72}
\\
$\scriptstyle \widetilde{\chi}^0_1\;\widetilde{\chi}^0_1$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle W^+\;W^-$ & $\scriptstyle 1412$ 
 & {\scriptsize 0.00586} & {\scriptsize 0.00585} & {\scriptsize 0.00586}
 & {\scriptsize 0.00586} & {\scriptsize 0.00587} & {\scriptsize 0.00586}
\\\hline
$\scriptstyle c\;\bar{s}$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle \widetilde{\chi}^0_1\;\widetilde{\chi}_1^+$ & $\scriptstyle 1114$ 
 & {\scriptsize 0.000873} & {\scriptsize 0.000874} & {\scriptsize 0.000873}
 & {\scriptsize 0.000873} & {\scriptsize 0.000874} & {\scriptsize 0.000873}
\\
$\scriptstyle \widetilde{\chi}^0_2\;\widetilde{\chi}^0_2$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle \widetilde{\chi}^0_2\;\widetilde{\chi}^0_2$ & $\scriptstyle 2897$ 
 & {\scriptsize 0.00237} & {\scriptsize 0.00237} & {\scriptsize 0.00237}
 & {\scriptsize 0.00237} & {\scriptsize 0.00236} & {\scriptsize 0.00237}
\\
$\scriptstyle \widetilde{\chi}_1^+\;\widetilde{\chi}_2^+$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle \widetilde{\chi}_2^+\;\widetilde{\chi}_2^+$ & $\scriptstyle 5286$ 
 & {\scriptsize 0.0151} & {\scriptsize 0.0151} & {\scriptsize 0.0151}
 & {\scriptsize 0.0151} & {\scriptsize 0.0151} & {\scriptsize 0.0151}
\\
$\scriptstyle c\;\bar{c}$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle \widetilde{\chi}^0_2\;\widetilde{\chi}^0_3$ & $\scriptstyle 2179$ 
 & {\scriptsize 0.000134} & {\scriptsize 0.000134} & {\scriptsize 0.000134}
 & {\scriptsize 0.000134} & {\scriptsize 0.000134} & {\scriptsize 0.000134}
\\
$\scriptstyle s\;\bar{s}$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle \widetilde{g}\;\widetilde{g}$ & $\scriptstyle 4862$ 
 & {\scriptsize 0.144} & {\scriptsize 0.144} & {\scriptsize 0.144} & {\scriptsize 0.144}
 & {\scriptsize 0.144} & {\scriptsize 0.144}
\\
$\scriptstyle \mu^-\;\mu^+$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle \widetilde{\chi}^0_2\;\widetilde{\chi}^0_2$ & $\scriptstyle 1449$ 
 & {\scriptsize 0.0291} & {\scriptsize 0.0291} & {\scriptsize 0.0291}
 & {\scriptsize 0.0291} & {\scriptsize 0.0291} & {\scriptsize 0.0291}
\\
$\scriptstyle t\;\bar{b}$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle \widetilde{\chi}^0_3\;\widetilde{\chi}_2^+$ & $\scriptstyle 3694$ 
 & {\scriptsize 0.00759} & {\scriptsize 0.00759} & {\scriptsize 0.00758}
 & {\scriptsize 0.00759} & {\scriptsize 0.00759} & {\scriptsize 0.00759}
\\
$\scriptstyle c\;\bar{c}$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle \widetilde{g}\;\widetilde{g}$ & $\scriptstyle 4862$ 
 & {\scriptsize 0.144} & {\scriptsize 0.144} & {\scriptsize 0.144} & {\scriptsize 0.144}
 & {\scriptsize 0.144} & {\scriptsize 0.144}
\\\hline
$\scriptstyle \tau^-\;u$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle \tilde{l}_6^-\;\tilde{u}_5$ & $\scriptstyle 3079$ 
 & {\scriptsize 0.000510} & {\scriptsize 0.000510} & {\scriptsize 0.000510}
 & {\scriptsize 0.000510} & {\scriptsize 0.000510} & {\scriptsize 0.000510}
\\
$\scriptstyle \nu_\mu\;\nu_\tau$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle \tilde{\nu}_1\;\tilde{\nu}_2$ & $\scriptstyle 1480$ 
 & {\scriptsize 0.00902} & {\scriptsize 0.00903} & {\scriptsize 0.00902}
 & {\scriptsize 0.00902} & {\scriptsize 0.00903} & {\scriptsize 0.00902}
\\
$\scriptstyle \gamma\;Z$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle \tilde{l}_1^-\;\tilde{l}_6^+$ & $\scriptstyle 1730$ 
 & {\scriptsize 0.00278} & {\scriptsize 0.00278} & {\scriptsize 0.00278}
 & {\scriptsize 0.00278} & {\scriptsize 0.00278} & {\scriptsize 0.00278}
\\
$\scriptstyle s\;\widetilde{\chi}^0_2$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle \tilde{d}_3\;H_1$ & $\scriptstyle 3349$ 
 & {\scriptsize 9.85e-06} & {\scriptsize 9.85e-06} & {\scriptsize 9.85e-06}
 & {\scriptsize 9.85e-06} & {\scriptsize 9.85e-06} & {\scriptsize 9.85e-06}
\\
$\scriptstyle \gamma\;Z$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle \tilde{u}_5\;\tilde{u}^*_5$ & $\scriptstyle 4854$ 
 & {\scriptsize 0.00268} & {\scriptsize 0.00268} & {\scriptsize 0.00268}
 & {\scriptsize 0.00268} & {\scriptsize 0.00268} & {\scriptsize 0.00268}
\\
$\scriptstyle \nu_e\;e^-$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle \tilde{\nu}_3\;\tilde{l}_2^-$ & $\scriptstyle 1317$ 
 & {\scriptsize 0.0274} & {\scriptsize 0.0274} & {\scriptsize 0.0274}
 & {\scriptsize 0.0274} & {\scriptsize 0.0274} & {\scriptsize 0.0274}
\\
$\scriptstyle s\;\widetilde{\chi}^0_1$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle \tilde{u}_4\;H^-$ & $\scriptstyle 4263$ 
 & {\scriptsize 9.84e-06} & {\scriptsize 9.84e-06} & {\scriptsize 9.84e-06}
 & {\scriptsize 9.84e-06} & {\scriptsize 9.84e-06} & {\scriptsize 9.83e-06}
\\
$\scriptstyle \tau^-\;\tau^+$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle \tilde{u}_1\;\tilde{u}^*_6$ & $\scriptstyle 3956$ 
 & {\scriptsize 0.000449} & {\scriptsize 0.000449} & {\scriptsize 0.000449}
 & {\scriptsize 0.000449} & {\scriptsize 0.000449} & {\scriptsize 0.000449}
\\\hline
\end{tabular}


==> table_sm.tex <==
\begin{tabular}{|lcl|l|lllllll|lll|}
\hline & & & & \multicolumn{7}{|c|}{\sc FeynRules} & \multicolumn{3}{|c|}{Stock}\\
\multicolumn{3}{|c|}{Process} & \multicolumn{1}{|c|}{$\sqrt{s}$}
 & \multicolumn{1}{|c}{CH} & \multicolumn{1}{c}{CH} & \multicolumn{1}{c}{MG}
 & \multicolumn{1}{c}{WO1} & \multicolumn{1}{c}{WO1} & \multicolumn{1}{c}{WO2}
 & \multicolumn{1}{c|}{WO2} & \multicolumn{1}{|c}{CH} & \multicolumn{1}{c}{MG}
 & \multicolumn{1}{c|}{WO2}\\
& & & \multicolumn{1}{c}{\scriptsize[GeV]} & \multicolumn{1}{|c}{F}
 & \multicolumn{1}{c}{U} & \multicolumn{1}{c}{U} & \multicolumn{1}{c}{F}
 & \multicolumn{1}{c}{U} & \multicolumn{1}{c}{F} & \multicolumn{1}{c|}{U}
 & \multicolumn{1}{|c}{U} & \multicolumn{1}{c}{U} & \multicolumn{1}{c|}{U}\\
\hline\hline
$\scriptstyle W^+\;W^+$ & $\scriptstyle\rightarrow$ & $\scriptstyle W^+\;W^+$ &
 $\scriptstyle 1277$ 
 & {\scriptsize 25.7} & {\scriptsize 25.7} & {\scriptsize 25.7} & {\scriptsize 25.7}
 & {\scriptsize 25.7} & {\scriptsize 25.7} & {\scriptsize 25.7} & {\scriptsize 25.7}
 & {\scriptsize 25.7} & {\scriptsize 25.7}
\\
$\scriptstyle g\;g$ & $\scriptstyle\rightarrow$ & $\scriptstyle g\;g$ &
 $\scriptstyle 200$ 
 & {\scriptsize 1.88e04} & {\scriptsize 1.88e04} & {\scriptsize 1.89e04}
 & {\scriptsize 1.88e04} & {\scriptsize 1.88e04} & {\scriptsize 1.88e04}
 & {\scriptsize 1.88e04} & {\scriptsize 1.88e04} & {\scriptsize 1.88e04}
 & {\scriptsize 1.88e04}
\\
$\scriptstyle Z\;Z$ & $\scriptstyle\rightarrow$ & $\scriptstyle W^+\;W^-$ &
 $\scriptstyle 1368$ 
 & {\scriptsize 26.2} & {\scriptsize 26.2} & {\scriptsize 26.2} & {\scriptsize 26.2}
 & {\scriptsize 26.2} & {\scriptsize 26.2} & {\scriptsize 26.2} & {\scriptsize 26.2}
 & {\scriptsize 26.2} & {\scriptsize 26.2}
\\
$\scriptstyle \gamma\;\gamma$ & $\scriptstyle\rightarrow$ & $\scriptstyle W^+\;W^-$ &
 $\scriptstyle 639$ 
 & {\scriptsize 16.3} & {\scriptsize 16.3} & {\scriptsize 16.3} & {\scriptsize 16.3}
 & {\scriptsize 16.3} & {\scriptsize 16.3} & {\scriptsize 16.3} & {\scriptsize 16.3}
 & {\scriptsize 16.3} & {\scriptsize 16.3}
\\
$\scriptstyle Z\;Z$ & $\scriptstyle\rightarrow$ & $\scriptstyle Z\;Z$ &
 $\scriptstyle 1459$ 
 & {\scriptsize 0.245} & {\scriptsize 0.245} & {\scriptsize 0.245} & {\scriptsize 0.245}
 & {\scriptsize 0.245} & {\scriptsize 0.245} & {\scriptsize 0.245} & {\scriptsize 0.245}
 & {\scriptsize 0.245} & {\scriptsize 0.245}
\\
$\scriptstyle \gamma\;Z$ & $\scriptstyle\rightarrow$ & $\scriptstyle W^+\;W^-$ &
 $\scriptstyle 1003$ 
 & {\scriptsize 19.3} & {\scriptsize 19.3} & {\scriptsize 19.3} & {\scriptsize 19.3}
 & {\scriptsize 19.3} & {\scriptsize 19.3} & {\scriptsize 19.3} & {\scriptsize 19.3}
 & {\scriptsize 19.3} & {\scriptsize 19.3}
\\\hline
$\scriptstyle s\;\bar{s}$ & $\scriptstyle\rightarrow$ & $\scriptstyle Z\;Z$ &
 $\scriptstyle 730$ 
 & {\scriptsize 0.0838} & {\scriptsize 0.0838} & {\scriptsize 0.0839}
 & {\scriptsize 0.0838} & {\scriptsize 0.0838} & {\scriptsize 0.0838}
 & {\scriptsize 0.0838} & {\scriptsize 0.0838} & {\scriptsize 0.0839}
 & {\scriptsize 0.0838}
\\
$\scriptstyle \mu^-\;\mu^+$ & $\scriptstyle\rightarrow$ & $\scriptstyle \gamma\;Z$ &
 $\scriptstyle 366$ 
 & {\scriptsize 1.46} & {\scriptsize 1.46} & {\scriptsize 1.46} & {\scriptsize 1.46}
 & {\scriptsize 1.46} & {\scriptsize 1.46} & {\scriptsize 1.46} & {\scriptsize 1.46}
 & {\scriptsize 1.46} & {\scriptsize 1.46}
\\
$\scriptstyle s\;\bar{s}$ & $\scriptstyle\rightarrow$ & $\scriptstyle \gamma\;\gamma$ &
 $\scriptstyle 200$ 
 & {\scriptsize 0.0272} & {\scriptsize 0.0272} & {\scriptsize 0.0272}
 & {\scriptsize 0.0272} & {\scriptsize 0.0272} & {\scriptsize 0.0272}
 & {\scriptsize 0.0272} & {\scriptsize 0.0272} & {\scriptsize 0.0272}
 & {\scriptsize 0.0272}
\\
$\scriptstyle u\;\bar{d}$ & $\scriptstyle\rightarrow$ & $\scriptstyle Z\;W^+$ &
 $\scriptstyle 684$ 
 & {\scriptsize 0.146} & {\scriptsize 0.146} & {\scriptsize 0.146} & {\scriptsize 0.146}
 & {\scriptsize 0.146} & {\scriptsize 0.146} & {\scriptsize 0.146} & {\scriptsize 0.146}
 & {\scriptsize 0.146} & {\scriptsize 0.146}
\\
$\scriptstyle c\;\bar{c}$ & $\scriptstyle\rightarrow$ & $\scriptstyle g\;g$ &
 $\scriptstyle 200$ 
 & {\scriptsize 462} & {\scriptsize 462} & {\scriptsize 462} & {\scriptsize 462}
 & {\scriptsize 462} & {\scriptsize 462} & {\scriptsize 462} & {\scriptsize 462}
 & {\scriptsize 462} & {\scriptsize 462}
\\
$\scriptstyle \nu_e\;e^+$ & $\scriptstyle\rightarrow$ & $\scriptstyle \gamma\;W^+$ &
 $\scriptstyle 319$ 
 & {\scriptsize 1.98} & {\scriptsize 1.98} & {\scriptsize 1.98} & {\scriptsize 1.98}
 & {\scriptsize 1.98} & {\scriptsize 1.98} & {\scriptsize 1.99} & {\scriptsize 1.98}
 & {\scriptsize 1.98} & {\scriptsize 1.98}
\\
$\scriptstyle d\;\bar{d}$ & $\scriptstyle\rightarrow$ & $\scriptstyle \gamma\;Z$ &
 $\scriptstyle 365$ 
 & {\scriptsize 0.0798} & {\scriptsize 0.0798} & {\scriptsize 0.0799}
 & {\scriptsize 0.0798} & {\scriptsize 0.0798} & {\scriptsize 0.0798}
 & {\scriptsize 0.0798} & {\scriptsize 0.0798} & {\scriptsize 0.0798}
 & {\scriptsize 0.0798}
\\
$\scriptstyle b\;\bar{b}$ & $\scriptstyle\rightarrow$ & $\scriptstyle Z\;Z$ &
 $\scriptstyle 767$ 
 & {\scriptsize 0.0760} & {\scriptsize 0.0760} & {\scriptsize 0.0758}
 & {\scriptsize 0.0760} & {\scriptsize 0.0760} & {\scriptsize 0.0760}
 & {\scriptsize 0.0760} & {\scriptsize 0.0760} & {\scriptsize 0.0758}
 & {\scriptsize 0.0760}
\\
$\scriptstyle c\;\bar{s}$ & $\scriptstyle\rightarrow$ & $\scriptstyle \gamma\;W^+$ &
 $\scriptstyle 325$ 
 & {\scriptsize 0.208} & {\scriptsize 0.208} & {\scriptsize 0.208} & {\scriptsize 0.207}
 & {\scriptsize 0.208} & {\scriptsize 0.208} & {\scriptsize 0.208} & {\scriptsize 0.208}
 & {\scriptsize 0.208} & {\scriptsize 0.208}
\\
$\scriptstyle \nu_\tau\;\bar{\nu}_\tau$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle W^+\;W^-$ & $\scriptstyle 639$ 
 & {\scriptsize 1.06} & {\scriptsize 1.06} & {\scriptsize 1.06} & {\scriptsize 1.06}
 & {\scriptsize 1.06} & {\scriptsize 1.06} & {\scriptsize 1.06} & {\scriptsize 1.06}
 & {\scriptsize 1.06} & {\scriptsize 1.06}
\\\hline
$\scriptstyle \nu_\mu\;\bar{\nu}_\tau$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle \mu^-\;\tau^+$ & $\scriptstyle 200$ 
 & {\scriptsize 16.5} & {\scriptsize 16.5} & {\scriptsize 16.5} & {\scriptsize 16.5}
 & {\scriptsize 16.5} & {\scriptsize 16.5} & {\scriptsize 16.5} & {\scriptsize 16.5}
 & {\scriptsize 16.5} & {\scriptsize 16.5}
\\
$\scriptstyle \nu_\mu\;\bar{\nu}_\mu$ & $\scriptstyle\rightarrow$ &
 $\scriptstyle \mu^-\;\mu^+$ & $\scriptstyle 200$ 
 & {\scriptsize 22.4} & {\scriptsize 22.4} & {\scriptsize 22.4} & {\scriptsize 22.4}
 & {\scriptsize 22.4} & {\scriptsize 22.4} & {\scriptsize 22.4} & {\scriptsize 22.4}
 & {\scriptsize 22.4} & {\scriptsize 22.4}
\\
$\scriptstyle t\;\bar{t}$ & $\scriptstyle\rightarrow$ & $\scriptstyle s\;\bar{s}$ &
 $\scriptstyle 1395$ 
 & {\scriptsize 1.14} & {\scriptsize 1.14} & {\scriptsize 1.14} & {\scriptsize 1.14}
 & {\scriptsize 1.14} & {\scriptsize 1.14} & {\scriptsize 1.14} & {\scriptsize 1.14}
 & {\scriptsize 1.14} & {\scriptsize 1.14}
\\
$\scriptstyle e^-\;e^+$ & $\scriptstyle\rightarrow$ & $\scriptstyle t\;\bar{t}$ &
 $\scriptstyle 1394$ 
 & {\scriptsize 0.0723} & {\scriptsize 0.0723} & {\scriptsize 0.0724}
 & {\scriptsize 0.0723} & {\scriptsize 0.0723} & {\scriptsize 0.0723}
 & {\scriptsize 0.0723} & {\scriptsize 0.0723} & {\scriptsize 0.0723}
 & {\scriptsize 0.0723}
\\
$\scriptstyle c\;c$ & $\scriptstyle\rightarrow$ & $\scriptstyle c\;c$ &
 $\scriptstyle 200$ 
 & {\scriptsize 3.41e03} & {\scriptsize 3.41e03} & {\scriptsize 3.42e03}
 & {\scriptsize 3.41e03} & {\scriptsize 3.41e03} & {\scriptsize 3.42e03}
 & {\scriptsize 3.41e03} & {\scriptsize 3.41e03} & {\scriptsize 3.41e03}
 & {\scriptsize 3.42e03}
\\
$\scriptstyle u\;\bar{u}$ & $\scriptstyle\rightarrow$ & $\scriptstyle s\;\bar{s}$ &
 $\scriptstyle 200$ 
 & {\scriptsize 80.3} & {\scriptsize 80.3} & {\scriptsize 80.2} & {\scriptsize 80.3}
 & {\scriptsize 80.3} & {\scriptsize 80.3} & {\scriptsize 80.3} & {\scriptsize 80.3}
 & {\scriptsize 80.3} & {\scriptsize 80.3}
\\
$\scriptstyle u\;\bar{u}$ & $\scriptstyle\rightarrow$ & $\scriptstyle d\;\bar{d}$ &
 $\scriptstyle 200$ 
 & {\scriptsize 68.1} & {\scriptsize 68.1} & {\scriptsize 68.0} & {\scriptsize 68.1}
 & {\scriptsize 68.1} & {\scriptsize 68.1} & {\scriptsize 68.1} & {\scriptsize 68.1}
 & {\scriptsize 68.1} & {\scriptsize 68.0}
\\
$\scriptstyle u\;\bar{t}$ & $\scriptstyle\rightarrow$ & $\scriptstyle d\;\bar{b}$ &
 $\scriptstyle 716$ 
 & {\scriptsize 5.49} & {\scriptsize 5.49} & {\scriptsize 5.49} & {\scriptsize 5.49}
 & {\scriptsize 5.49} & {\scriptsize 5.49} & {\scriptsize 5.49} & {\scriptsize 5.49}
 & {\scriptsize 5.50} & {\scriptsize 5.49}
\\
$\scriptstyle \nu_\tau\;\tau^+$ & $\scriptstyle\rightarrow$ & $\scriptstyle u\;\bar{s}$ &
 $\scriptstyle 200$ 
 & {\scriptsize 0.501} & {\scriptsize 0.501} & {\scriptsize 0.501} & {\scriptsize 0.501}
 & {\scriptsize 0.501} & {\scriptsize 0.501} & {\scriptsize 0.501} & {\scriptsize 0.501}
 & {\scriptsize 0.501} & {\scriptsize 0.501}
\\
$\scriptstyle \nu_\mu\;\mu^+$ & $\scriptstyle\rightarrow$ & $\scriptstyle c\;\bar{s}$ &
 $\scriptstyle 200$ 
 & {\scriptsize 9.33} & {\scriptsize 9.33} & {\scriptsize 9.32} & {\scriptsize 9.33}
 & {\scriptsize 9.33} & {\scriptsize 9.33} & {\scriptsize 9.33} & {\scriptsize 9.33}
 & {\scriptsize 9.33} & {\scriptsize 9.33}
\\\hline
$\scriptstyle Z\;Z$ & $\scriptstyle\rightarrow$ & $\scriptstyle H\;H$ &
 $\scriptstyle 1690$ 
 & {\scriptsize 0.250} & {\scriptsize 0.250} & {\scriptsize 0.250} & {\scriptsize 0.250}
 & {\scriptsize 0.250} & {\scriptsize 0.250} & {\scriptsize 0.250} & {\scriptsize 0.250}
 & {\scriptsize 0.250} & {\scriptsize 0.250}
\\
$\scriptstyle W^+\;W^-$ & $\scriptstyle\rightarrow$ & $\scriptstyle H\;H$ &
 $\scriptstyle 1599$ 
 & {\scriptsize 0.151} & {\scriptsize 0.151} & {\scriptsize 0.151} & {\scriptsize 0.151}
 & {\scriptsize 0.151} & {\scriptsize 0.151} & {\scriptsize 0.151} & {\scriptsize 0.151}
 & {\scriptsize 0.151} & {\scriptsize 0.151}
\\
$\scriptstyle t\;\bar{t}$ & $\scriptstyle\rightarrow$ & $\scriptstyle H\;H$ &
 $\scriptstyle 2354$ 
 & {\scriptsize 0.0593} & {\scriptsize 0.0593} & {\scriptsize 0.0593}
 & {\scriptsize 0.0593} & {\scriptsize 0.0593} & {\scriptsize 0.0593}
 & {\scriptsize 0.0593} & {\scriptsize 0.0593} & {\scriptsize 0.0593}
 & {\scriptsize 0.0593}
\\
$\scriptstyle \tau^-\;\tau^+$ & $\scriptstyle\rightarrow$ & $\scriptstyle H\;H$ &
 $\scriptstyle 974$ 
 & {\scriptsize 2.96e-06} & {\scriptsize 2.96e-06} & {\scriptsize 2.96e-06}
 & {\scriptsize 2.96e-06} & {\scriptsize 2.96e-06} & {\scriptsize 2.96e-06}
 & {\scriptsize 2.96e-06} & {\scriptsize 2.96e-06} & {\scriptsize 2.96e-06}
 & {\scriptsize 2.96e-06}
\\
$\scriptstyle b\;\bar{b}$ & $\scriptstyle\rightarrow$ & $\scriptstyle H\;H$ &
 $\scriptstyle 998$ 
 & {\scriptsize 6.33e-06} & {\scriptsize 6.33e-06} & {\scriptsize 6.33e-06}
 & {\scriptsize 6.33e-06} & {\scriptsize 6.33e-06} & {\scriptsize 6.33e-06}
 & {\scriptsize 6.33e-06} & {\scriptsize 6.33e-06} & {\scriptsize 6.33e-06}
 & {\scriptsize 6.33e-06}
\\\hline
\end{tabular}

